Vision Transformer Computation and Resilience for Dynamic Inference

State-of-the-art deep learning models for computer vision tasks are based on the transformer architecture and often deployed in real-time applications. In this scenario, the resources available for every inference can vary, so it is useful to be able to dynamically adapt execution to trade accuracy for efficiency. To create dynamic models, we leverage the resilience of vision transformers to pruning and switch between different scaled versions of a model. Surprisingly, we find that most FLOPs are generated by convolutions, not attention. These relative FLOP counts are not a good predictor of GPU performance since GPUs have special optimizations for convolutions. Some models are fairly resilient and their model execution can be adapted without retraining, while all models achieve better accuracy with retraining alternative execution paths. These insights mean that we can leverage CNN accelerators and these alternative execution paths to enable efficient and dynamic vision transformer inference. Our analysis shows that leveraging this type of dynamic execution can lead to saving 28\% of energy with a 1.4\% accuracy drop for SegFormer (63 GFLOPs), with no additional training, and 53\% of energy for ResNet-50 (4 GFLOPs) with a 3.3\% accuracy drop by switching between pretrained Once-For-All models.

==> figures/figure_ofa_energy_per_flop.tex <==
\begin{figure}[t]

  \centering
  
  \includegraphics[width=1\linewidth]{images/img_ofa_energy_per_flop.png}

  \vspace{-0.05in}
  
  \caption{Normalized energy per FLOP for ofa-resnet50D-41 model layers with inference with a 224 by 224 image on accelerator E. %Highest energy is set to 1.
  }

\label{figure_ofa_energy_per_flop}
  
  \vspace{-0.1in}
 
\end{figure}


==> figures/figure_segformer_pareto.tex <==
\begin{figure}[t]

  \centering
  
  \includegraphics[width=1\linewidth]{images/img_segformer_pareto.png}
  \caption{Tradeoff between execution time, energy, and mIoU when dynamically pruning pretrained SegFormer B2 models on the A5000 GPU and accelerator E. Dynamic configuration labels have the four encoder stages depths and input channels for \textit{Conv2DFuse} and \textit{Conv2DPred} (values changed from original model are underlined).
  }
  
  \label{figure_segformer_pareto}
  
  % \vspace{-0.2in}
 
\end{figure}


==> figures/figure_swin_energy_per_flop.tex <==
\begin{figure}[t]

  \centering
  
  \includegraphics[width=1\linewidth]{images/img_swin_energy_per_flop.png}

  \vspace{-0.05in}
  
  \caption{Normalized energy per FLOP for Swin Tiny model layers with inference with a 512 by 512 image on accelerator E. %Highest energy is set to 1.
  }

\label{figure_swin_energy_per_flop}
  
  \vspace{-0.1in}
 
\end{figure}


==> figures/figure_throughput_area_energy_all.tex <==
\begin{figure*}[t]

  \centering
  
  \includegraphics[width=1\linewidth]{images/img_throughput_area_energy_all.png}

  \vspace{-0.05in}
  
  \caption{Energy per FLOP vs throughput per area for SegFormer ADE B2, Swin Tiny, and OFA-resnet50D-41 for accelerators in Table~\ref{table_accelerator_configs}. Swin Tiny does not include A and C since they were not competitive from SegFormer ADE B2, while OFA-resnet50D-41 does not include K0 = C0 = 16 accelerators since they were not competitive from SegFormer ADE B2 and Swin Tiny.
  }
  
  \label{figure_throughput_area_energy_all}
  
  \vspace{-0.15in}
 
\end{figure*}

